NARRATE: A Normal Assisted Free-View Portrait Stylizer

In this work, we propose NARRATE, a novel pipeline that enables simultaneously editing portrait lighting and perspective in a photorealistic manner. As a hybrid neural-physical face model, NARRATE leverages complementary benefits of geometry-aware generative approaches and normal-assisted physical face models. In a nutshell, NARRATE first inverts the input portrait to a coarse geometry and employs neural rendering to generate images resembling the input, as well as producing convincing pose changes. However, inversion step introduces mismatch, bringing low-quality images with less facial details. As such, we further estimate portrait normal to enhance the coarse geometry, creating a high-fidelity physical face model. In particular, we fuse the neural and physical renderings to compensate for the imperfect inversion, resulting in both realistic and view-consistent novel perspective images. In relighting stage, previous works focus on single view portrait relighting but ignoring consistency between different perspectives as well, leading unstable and inconsistent lighting effects for view changes. We extend Total Relighting to fix this problem by unifying its multi-view input normal maps with the physical face model. NARRATE conducts relighting with consistent normal maps, imposing cross-view constraints and exhibiting stable and coherent illumination effects. We experimentally demonstrate that NARRATE achieves more photorealistic, reliable results over prior works. We further bridge NARRATE with animation and style transfer tools, supporting pose change, light change, facial animation, and style transfer, either separately or in combination, all at a photographic quality. We showcase vivid free-view facial animations as well as 3D-aware relightable stylization, which help facilitate various AR/VR applications like virtual cinematography, 3D video conferencing, and post-production.

==> section/depre/Introduction-v2.tex <==
\section{Introduction}



\begin{comment}
Even in today's digital era, portrait photography remains inarguably the most popular photography genre. For any successful portrait, be it a corporate headshot, a beauty shot, or a character study, lighting styles, coupled with shooting angles, play the key role to emphasize the subject's feature as well as to express artistic or dramatic intent. For example, popular loop lighting defines facial features with soft shadows to illustrate harmony whereas a half lit and half in shadow face by split lighting reflects the subject's inner struggle. Rambrandt pioneered combining a key light and a fill light (e.g., a reflector) to construct a distinctive triangle of light on one cheek, baking a moody atmosphere.

Despite rich diversities in styles, a portrait, once taken, is fixed in its appearance where post-capture lighting alteration remains difficult, let alone complete lighting style changes. Perspective changes, in contrast, have attracted much attention in both computer vision and computer graphics communities. the main idea is to rig the portrait [], with or without explicitly modeling facial geometry. Classic 3D morphable face model (3DMM) XXX. Extensions. Rely on high quality scans. Generation approaches. StyleGAN XXX.

The seminal work of StyleSDF. combine generation with explicit geometry constraints. Describe how it works. How to use it to realize lighting style changes. Limitations: 1) a generation task, cannot fix the subject, unless inversion. inversion not reliable with appearance only. 2) geometry quality not sufficient for lighting. 

Our approach. 1), 2), 3), 4). 

Experimental validations. Applications. Beyond light stylization with availability of normal.

Jingyi's structure
I. Intro
1. Portrait stylization. Reconstruction tasks vs. Generation tasks. Former: relighting but not free viewpoint; core techniques; Latter: cannot enable photorealistic relighting; 
2. Existing approaches. Model-based: issues, cannot model hair and ears, let alone clothing, parametric model + texture mapping still lacks realism due to incorrect shape and lack of view dependencies; StyleSDF geometry not sufficient (discuss SIG paper this year). 
3. Our approach. Core: dataset augmentation; 
4. Applications: 1) Non-photorealistic rendering; 2) Super-resolution?? 3) Simultaneous relighting + perspective adjustment; 
5. Generation tasks: normal map adjustment/transfer - why for what purpose? detail preservation transfer (wrinkles?); aging and deaging. 
\end{comment}

\begin{comment}
\wz{It is a pipeline paper, where we propose a free view, relightable pipeline for poitraint stylization.

1) portrait photography is popular. lighting and view angle is important.
2) post process is hard--> we want to jointly edit view, light at high quality. no existing works achieve all three goals.
3) existing relighting works xxx
4) existing perspective changing works xxx -> 3DMM, generation
5) geometry aware generative models xxx
6) our solution -> fulfill all the requirements.
7) its free view editing is enhanced with normal
8) its lighting module xxx
9) its application supports magic photo in harry potter and palace opera solo animation
10) summary.
%3) a new way: 3D aware generative models can help but still limited
%4) our approach.
}
\end{comment}

% 1) portrait photography is popular, lighting are important.
Even in today's digital era, portrait photography remains inarguably the most popular genre. 
For any successful portrait, be it an actor still, a beauty shot, or a character study, \emph{lighting styles}, coupled with \emph{shooting angles}\wz{need a unified definition}, play the key role to emphasize the subject's feature as well as to express artistic or dramatic intent. On lighting, popular loop lighting defines facial features with soft shadows to illustrate harmony whereas a half lit and half in shadow face by split lighting reflects the subject's inner struggle. Rambrandt lighting combines a key light and a fill light (e.g., a reflector) to cast a distinctive triangle of light on one cheek, baking a moody atmosphere. On shooting angle, front view (full face) shots highlight complete facial details to convey an assertive attitude whereas side view (profile) shots emphasize on the physical form-factor such as facial contours to exude character. Three-quarter views, popularized by self-portraits, reveal both with a personal touch. 

%different portrait styles need to be captured under specific viewing angles. 
%portrait shooting angles also strongly influence the artistic effects. E.g., an ID photo requires front view to describe the whole face characteristic while a beauty shot prefers side view to better present appealing face features as well as harmonically blend into the background.
\wz{the current starting focuses too much on relighting, say sth with view angles.}

% 1) editting photography is still hard
Despite richness in styles, a portrait, once taken, is fixed in its final presentation. Style changes, even though highly desirable, remains largely unresolved even with the most advanced retouching tools. The challenges are multi-fold. Persuasive lighting adjustment requires reliable estimations of a portrait's original illumination and detailed facial geometry, e.g., normals. Further, high photorealism needs to be maintained under perspective changes where existing warping-based techniques still fall short of.  In this paper, we present a novel neural portrait stylization pipeline that can simultaneously edit a portrait's \textbf{lighting effects} and \textbf{shooting angles} at the \textbf{photographic} quality, benefiting photographers and visual artists as well as daily users. Our pipeline can be further extended to produce styled facial animations to support virtual cinematography, post-production, tele-presence, etc. 

%task remains difficult. Prior works have focused on one or two aspects of the above requirements, but no existing method fulfills all of them. 

Most existing portrait relighting works are designed for fixed input view~\cite{} which cannot be applied in free view lighting alteration. Recent works~\cite{} combine relighting and view editing together, but xxx. As a consequence, they cannot support high quality realistic view editing, let alone complete lighting style changes. 
\wz{say sth more about the limitation about light changes. @XULAN What's the other work that support free view relighting?} 


Portrait perspective changes, in contrast, have a much longer history in both computer graphics and computer vision. The most widely adopted solution so far is to rig the portrait, either with or without explicitly modeling facial geometry. 
% Classic 3D morphable face model (3DMM) methods~\cite{} build statistics PCA models to represent 3D facial shape and texture in low dimension PCA coefficients. to the images. Once trained, it can further be used to represent the 3D model. 
The former largely adopts 3D morphable models (3DMM)~\cite{}, which represent 3D face by statistics PCA models. 
Recent neural network based 3DMM methods are able to predict faithful shape and texture, and render them in novel views.
However, 3DMM models focus overwhelmingly on large scale geometry of face and tend to produce overly smooth surfaces that lack details. They are also sensitive to corner cases, such as various hair styles, wrinkled clothes, topological changes caused by glasses or even ears. The quality of the final rigged result cannot yet match the original photography. 
% Other variants~\cite{} rely on high quality scans, which are not suitable for single view portrait perspective editing either.
% 2D gans
Implicit solutions, popularized by generative models~\cite{gan, stylegan123}, have shown potential for high quality portrait synthesis. Their goal is not to change the style of an existing portrait but to create various styles by manipulating the latent space. The seminal XXX framework [] produces perspective variations by XXX ~\cite{}. Yet, the lack of geometric constraints prohibits it from producing convincing perspective changes where the results exhibit strong aliasing and inconsistency. Recent geometry-aware generative models~\cite{pigan,ed3d,stylesdf} combine 2D generation with explicit 3D geometry constraints and have shown stunning successes. 
They map latent codes to 3D representations~\cite{} and leverage differentiable rendering to convert 3D representations back to 2D images to avoid 3D supervision~\cite{}. These techniques can achieve much higher view consistency in perspective changes but their target is still generation rather than stylizing an existing portrait. They also rely mainly on coarse geometry for training where the high resolution is achieved via CNN upsampling, causing vibration artifacts across views. Further, the quality of geometry is not readily sufficient for relighting. 


\wz{do we mention volux gan here or in related work? we mention in related work. Say In current work, XXX et al. XXX}
Consequently, it is hard to apply them in free-view relighting, either.


%How to use it to realize lighting style changes. Limitations: 1) a generation task, cannot fix the subject, unless inversion. inversion not reliable with appearance only. 2) geometry quality not sufficient for lighting.

\wz{Current version is too verbose. Need condense them into half. Some of them will put in related work. Also, we focus on the view changes methods, we should talk more about lighting.}

\wz{we can consider submit to neurips :). The name is just for fun.}
In this work, we introduce {\ourmodel}(Normal Enhanced neURal Implicit surfaces for Portrait Stylization), a novel \wz{can we use novel?} pipeline that fulfills all the requirements of portrait stylization.  From a front view \wz{can we do other view?} portrait as input, {\ourmodel} supports free-view lighting alteration and produces faithful editing effects at photography quality. We carefully design {\ourmodel} by combine a geometry aware generative model~\cite{} and a relighting network to achieve these goals. 

At its core, we first leverage StyleSDF to turn a 2D portrait into a 3D shape via inversion~\cite{} and produce a novel view image with neural rendering. 
To alleviate the fitting mismatch and vibrating artifacts, % introduced by inversion and neural rendering, 
we enhance the low quality geometry with a inferred normal map~\cite{}, creating a high fidelity textured mesh.
It is further passed through regular rendering engines~\cite{} and synthesize a new image full of realistic portrait details. We fuse the two renderings to generate a high-quality image with minimal artifacts at arbitrary views,  both for the main face region as well as for corner cases like hair, glass and clothes. 

We then stylize the lighting effects with the free view image. Inspired by xxx~\cite{}, we train a decomposition network to map it into albedo and normal maps. The intermediate results are sent to a synthesis network to create exquisite lighting effects with manually specified illumination conditions. We improve ~\cite{} by xxx\wz{can we do sth novel?}. Our method supports a wide range of complex lighting styles, producing realistic relighting effects as shown in the Fig.~\ref{fig:teaser}.

Beyond the high-quality free view relighting, {\ourmodel} can further be coupled with other facial applications to create movie special effects. We incorporate our pipeline with image stylization~\cite{} and facial animation~\cite{}. Such marriage brings dramatic reactions, allowing us to create delicate animations including magic photos in Harry Potter~\cite{} and vivid palace opera solo. {\ourmodel} has great potential to be applied in more scenarios to help artists create exquisite effects.
% Previously, they always require manual work and we first automatize it to reduce the burden of the artists.
%never achieved by any previous works.
% Nothing limits our pipeline has the potential to be applied to more applitiosn.

% I don;t think we need it... Now it is aleway very long
We summary our contributions as follow.
\begin{itemize}
  \item We propose {\ourmodel}, an automatic portrait stylization pipeline which enables high-quality, free view relighting.
  \item We demonstrate our normal enhanced solution largely reduces the free view editing artifacts, creating plausible and stable novel view synthesis. 
  \item Our light module xxx.
  \item We connect {\ourmodel} with stylization and ficial animation and showcase magic face editing effects.
\end{itemize}



\begin{comment}

Previous works address it in two lines: reconstruction and generation. 3D face reconstruction from  based methods. The former takes an 2D face image as input and predicts the corresponding xx and xx. 


Generating such video portraits conveniently still remains challenging and has attracted substantive attention of both the computer vision and graphics communities.
% with the rise of Virtual Reality (VR) and Augmented Reality (AR)

% 2. Issues of existing methods
In this paper, we focus on automatically and conveniently synthesizing a photo-realistic video portrait of a \textit{target} actor where the facial expression, the lighting condition and background are fully disentangled and controllable through various \textit{source} actors.
%
It is particularly challenging since humans are highly sensitive to facial inconsistency and the video portraits are influenced by the complex interaction of environment, lighting patterns and various facial attributes like material and specular reflection. 
% 2.1 Early movie industry, tedious manual labor and devices
The most common practice for manipulating video portraits in the film industry still relies on tedious manual labor and sophisticated devices for reflectance field acquisition~\cite{debevec2000acquiring} or chroma-keying~\cite{wright2006digital}.
% 2.2 Reenactment approach
The recent neural techniques~\cite{NR_survey,kim2018deep} bring huge potential for convenient and highly-realistic manipulations, enabling compelling visual quality in various applications, such as visual dubbing~\cite{kim2019neural,ji2021audio}, telepresence~\cite{lombardi2018deep}, video post-editing~\cite{fried2019text,yao2020talkinghead} or audio-driven virtual assistant~\cite{thies2020neural}, even in real-time~\cite{thies2016face2face,thies2018headon}.
%
However, they still suffer from pre-baked shading of the specific training scenes without manipulating the illumination, which is critical for relighting applications in portrait photography like virtual cinematography.
% 2.3 Relighting approach
On the other hand, various neural schemes with controllable portrait's lighting conditions have been proposed using high-quality pore-level 4D facial reflectance fields~\cite{debevec2000acquiring} acquired under multi-view and multi-lit configurations.
%
However, they are limited to image-based relighting~\cite{sun2019single,pandey2021total}, a subset of the reflectance field learning~\cite{sun2020light,meka2019deep} or relightable model and appearance reconstruction~\cite{guo2019relightables,meka2020deep,bi2021avatar}.
%
Researchers pay less attention to combine the background and lighting manipulation with face-interior reenactment into a universal data-driven framework.

% 3. Our key idea:
In this paper, we attack the above challenges and present the first approach to generating relightable neural video portraits for a specific performer. 
% 
As illustrated in Fig.~\ref{fig:teaser}, with the aid of immediate and high-quality facial reflectance field inference, our approach endows the entire photo-realistic video portraits synthesis with the ability of fully disentanglement and control of various head poses, facial expressions, backgrounds, and lighting conditions.
%
This unique capability also enables numerous photo-realistic visual editing effects.


% 4. Our technical pipeline
% Generating such photo-realistically editable neural video portraits in a data-driven manner is non-trivial.
% our key idea
Our key idea is to combine high-quality 4D reflectance field learning, model-based facial performance capture and target-aware neural rendering into a consistent framework, so as to support convenient, realistic and controllable editing of neural video portraits. 
% 4.1 Data-recording
To this end, for the temporal ground-truth supervision, we first build up a light stage setup to collect the dynamic facial reflectance fields of the target performer with one-light-at-a-time (OLAT) images under various sequential poses and expressions.
% 
%Our capture device consists of 96 LED light sources and a stationary 4K ultra-high-speed camera at 1000 fps, so as to provide fine-grained facial perception.
%
% 4.2 video-to-video translation
Then, with such target-specific OLAT data, the core of our approach is a novel rendering-to-video translation network design with the explicit head pose, facial expression, lighting and background disentanglement for highly controllable neural video portrait synthesis.
% %
% Specifically, our network takes the hybrid 2D and 3D model-based facial capture results as input, and generates corresponding high-quality OLAT imagesets as output.   
% %
% To enable reliable explicit control of the pose and expression, we carefully design a semantic-aware facial normalization scheme with a hierarchical landmark structure.
% %
% For high-quality reflectance field inference, we adopt a multi-task multi-frame learning framework, which not only jointly models the content and segmentation information using a hybrid loss design, but also encodes the rich temporal information in the captured dynamic OLAT dataset in a sliding window manner. 
% 4.3 edditable new effects 
After training, reliable head pose and facial expression editing are obtained by applying the same facial capture and normalization scheme to the source video input, while our explicit OLAT output enables high-quality relit effect. This relit effect can not only match the portrait with the environment, but also simulate the rim-light to improve the matting quality for a better background replacement.
%
An encoder-decoder architecture is further adopted to encode the illumination weighting parameters of OLAT images from the corresponding relit images, enabling automatic lighting editing from natural source images.
%
Thus, our approach enables automatically and conveniently control of facial expression, lighting condition and background of the performer's video portrait with high photo-realism for various visual editing effects.
% %
% More impressively, our approach can generate high frame-rate OLAT images (i.e, 1000 fps) for slow-motion relighting by interpolating the facial captured input of our translation network, which are regarded as extremely challenging using existing light stage devices due to the physical frame-rate constraint.
%5. Our technical contribution
To summarize, our main contributions include: 
\begin{itemize} 
	\setlength\itemsep{0em}
	\item We demonstrate the new capability of simultaneous relighting and and expression transfer, which enables photo-realistic video portraits synthesis for various visual editing effects, with full disentanglement of expressions, backgrounds and lighting conditions.
	
	\item We introduce a rendering-to-video translation network to transfer model-based input into high-fidelity facial reflectance fields, with a multi-frame multi-task learning strategy to encode content, segmentation and temporal information.
		
	\item We propose to utilize hybrid model-based facial capture with a carefully designed semantic-aware facial normalization scheme for reliable disentanglement.
	 
\end{itemize} 
\end{comment}

==> section/depre/Related_work-v0.tex <==
\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=0.93\linewidth]{fill_images/overview.png}
	\end{center}
	\vspace{-0.5cm}
	\caption{x xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xxx xxx xxxx xx xxxxx xx.}
	\label{fig:overview}
	\vspace{-0.3cm}
\end{figure*}


\section{Related Work}
\wz{3 parts: face }
\textbf{Face capture and reconstruction.}
 Face reconstruction methods aim to reconstruct the geometry and appearance of 3D face models from visual data and we refer to two recent reports on monocular 3D face reconstruction and applications~\cite{zollhofer2018state,egger20203d} for a comprehensive overview.
%
Early solutions adopt optimization schemes by fitting a 3D template model of only the face regions into various visual input, such as a single image~\cite{blanz2004exchanging,blanz1999morphable}, a temporal consistent video~\cite{cao2014displaced,fyffe2014driving,suwajanakorn2014total,ichim2015dynamic,garrido2016reconstruction,wu2016anatomically} or even unstructured image sets~\cite{kemelmacher2010being,kemelmacher2013internet,roth2016adaptive}.
%
The recent deep learning techniques bring huge potential for face modeling, which learn to predict the 3D face shape, geometry or appearance~\cite{kazemi2014one,zhu2017face,tewari2017mofa,tewari2018self,tewari2019fml,cao2015real,richardson20163d,richardson2017learning,yamaguchi2018high}
%
% Some recent work~\cite{booth2018large,li2017learning} learn a parametric face model from a large scale of 3D facial scans, while Feng~\emph{et al.}~\cite{feng2020learning} furthers model a parametric detail layer in a data-driven manner.
% %
% Some recent work also illustrates that a face parametric model can be trained from only image or video input~\cite{mallikarjun2020learning} or combining the implicit representation~\cite{yenamandra2020i3dmm}.
% %
However, these method above still cannot create a photo-realistic model in a controllable manner, especially for those fine-grained facial regions like hair, mouth interior or eye gaze.
% %
% Recent target-specific neural rendering techniques~\cite{lombardi2018deep,wei2019vr,bi2021avatar} further enable more realistic geometry and appearance reconstruction using the data captured under a multi-view and multi-lit configuration.
% %
% However, these neural models still heavily rely on per-frame facial geometry reconstruction during training and the final rendering results still suffer from reconstruction limitation and artifacts near the hair regions.
%
The recent work~\cite{gafni2020dynamic} enables controllable implicit facial modeling and rendering using neural radiance field,  but it still relies on per-scene training and suffers from pre-baked illumination of the training scenes.
%
In contrast, our approach enables more disentanglement and control of background, lighting condition as well as facial capture parameters for photo-realistic video portrait generation.


\textbf{Face reenactment and replacement.}
Facial reenactment re-generates the face content of a target actor in a portrait video by transferring facial expression and pose from a source actor.
%
Many recent reenactment approaches model-based expression capturing and the expressions are transferred via dense motion fields~\cite{liu2011realistic,suwajanakorn2015makes,averbuch2017bringing} or facial parameters~\cite{vlasic2006face,garrido2014automatic,li2013data,thies2015real,thies2016face2face,thies2018facevr}.
%
The recent neural approaches~\cite{NR_survey,kim2018deep} replace components of the standard graphics pipeline by learned components, which bring huge potential for convenient and highly-realistic manipulations, enabling compelling visual quality in various applications, such as visual dubbing~\cite{kim2019neural,ji2021audio}, telepresence~\cite{lombardi2018deep}, video post-editing~\cite{fried2019text,yao2020talkinghead} or audio-driven virtual assistant~\cite{thies2020neural}, even in real-time~\cite{thies2016face2face,thies2018headon}.
%
Inspired by pix2pix~\cite{isola2017image}, Deep Video Portraits~\cite{kim2018deep} proposes an rendering-to-image translation approach that converts synthetic rendering input to a scene-specific realistic image output. 
%
% The following work~\cite{kim2019neural} present reenactment to maintain the speaking style of the target identity by modeling the audio information for visual dubbing.
%
% The recent work~\cite{ji2021audio} further considers the emotion signal to generate target-specific emotional video portraits through only audio input.
%
% Besides, Deferred Neural Rendering~\cite{thies2019deferred} utilize neural textures to produce photo-realistic output, demonstrating high quality facial re-rendering and reenactment with the parametric 3D Morphable Model (3DMM) as input. 
%
% Recently, neural reenactment approaches~\cite{olszewski2016high,chung2017you,suwajanakorn2017synthesizing,thies2020neural,fried2019text} for video post-editing driven by audio or text have been widely explored.
%
% Specifically, Fried~\emph{et al.}~\cite{fried2019text} propose to map phonemes to the parameters of the 3DMM so as to smooth text-based reenactment.
%
% Thies~\emph{et al.}~\cite{thies2020neural} present Neural Voice Puppetry, which estimates parameters of a facial blendshape expression model from the audio logits followed by neural rendering for photo-realistic results. 
%
However, ~\cite{kim2018deep} and the work followed by, such as ~\cite{kim2019neural, ji2021audio, thies2019deferred}  suffers from pre-baked shading of the specific training scenes without manipulating the illumination which is critical for relighting applications like virtual cinematography.
%
Some recent work enables lighting or facial expression control during the facial portrait image generation~\cite{tewari2020stylerig,chen2020free} or editing~\cite{tewari2020pie,tewari2021photoapp} based on styleGAN~\cite{karras2019style}.
%
However, these methods mainly focus on the task of portrait image generation and suffers from unrealistic interpolation for neural video portrait reenactment.
%
Differently, we take advantage of learning from the temporally consistent OLAT dataset of the target performer to allow for larger changes in facial expression reenactment, background as well as the lighting condition, while maintaining high photo-realism.
%


\textbf{Facial portrait relighting.}
High quality facial portrait relighting requires the modeling of pore-level 4D reflectance fields.
%
Debevec~\emph{et al.}~\cite{debevec2000acquiring} invent Light Stage to capture the reflectance field of human faces, which has
enabled high-quality 3D face reconstruction and illuminations rendering, advancing the film’s special effects industry. 
%
Some subsequent work has also achieved excellent results by introducing deep learning~\cite{zhang2021neural,meka2019deep,meka2020deep,guo2019relightables,sun2019single}.
%
Some work follows the pipeline of color transfer to achieve the relighting effects~\cite{chen2011face,shih2014style,shu2017portrait,song2017stylizing}, which usually needs another portrait image as the facial color distribution reference. 
%
With the advent of deep neural networks and neural rendering, some methods~\cite{zhou2019deep,liu2021relighting,sengupta2018sfsnet} adopt Spherical Harmonics (SH) lighting model to manipulate the illumination. 
%
Several works~\cite{aldrian2012inverse,egger2018occlusion, wang2007face} jointly estimate the 3D face and SH [5, 34] parameters and achieved relighting by recovering the facial geometry and modify the parameters of the SH lighting model. 
%
Explicitly modeling the shadow and specular~\cite{wang2020single,nestmeyer2020learning} achieve excellent results in directional light source relighting. 
%
Mallikarjunr~\emph{et al.}~\cite{tewari2020monocular} take a single image portrait as input to predict OLAT(one-light-at-a-time) as Reflectance Fields, which can be relit to other lighting via image-based rendering. 
%
Sun~\emph{et al.}~\cite{sun2019single} choose environment map as lighting model and use light stage captured OLAT data to generate realistic training data and train relighting networks in an end-to-end fashion. 
%
Similarly, we use the target-aware temporal OLAT images to generate training data for high-quality lighting disentanglement.
%
Differently, we further combine the background and lighting manipulation with face-interior reenactment into a universal data-driven framework.

==> section/depre/abs_v1.tex <==

\begin{abstract}
	
	% our goal
	% limitation of previous work
	% our method
	% how do we do it
	% demonstration
	
	 Taking a compelling portrait photo relies on deliberately designed lighting effects and shooting angles, requiring advanced skills beyond ability of casual users. 
	%
	% Building a portrait stylization tool that supports both \emph{lighting} and \emph{perspective} adjustment at \emph{photographic quality} automate the editing process is beneficial to artists and daily users, enabling numerous applications from photography/cinematography to AR/VR. 
	Building a portrait stylization tool that automates lighting and perspective editing 
	% in post-processing 
	is beneficial to photographers and artists, enabling numerous applications from photography/cinematography to AR/VR. 
	%
	% This task remains challenging as most prior works address the two requirements separately,  handling either relighting or perspective changing alone. 
	This task remains challenging as \emph{persuasive lighting adjustment} and \emph{geometrically correct perspective changes} need to be addressed at the same time while still maintaining \emph{high photorealism}.
	%
	Naively bridging relighting and view synthesis methods %without considering their inherent connection
	produces inaccurate and unstable editing results.
	%
	In this work, we propose {\ourmodel}, a novel pipeline that enables photo-realistic portrait relighting and perspective editing simultaneously. 
	%
	It consists of a geometry aware generative model~\cite{orel2021styleSDF} to inverse the portrait to a latent code and generate desired novel view images, as well as a relighting network~\cite{pandey2021total} to modify their illuminations.
	%
	Instead of simply putting two models together, we tailor them for our task settings. 
	We observe that portrait geometry plays as key in both of them and propose to enhance their editing effects via normal information. 
	%
	Specifically, in novel view synthesis, images directly generated with inversion~\cite{orel2021styleSDF} fail to keep all facial details. We adopt normal maps to improve portrait geometry quality, creating new renderings from high-quality textured meshes and fusing them to compensate for the imperfect inversion, resulting in more realistic and detailed novel view images. 
	% we create and render high quality textured meshes from normal maps, fusing the generated images and rendered images .fails to keep all details
	%
	In relighting stage, ~\cite{pandey2021total} ignores consistency between different perspectives, leading unstable and inconsistent lighting effects. We strength it by unifying geometry under different views. Our relighting model takes uniform normal maps as input, exhibiting stable and consistent illuminations  %among various views.
	across different views.
	%
	We experimentally demonstrate that {\ourmodel} achieves % photorealism
	high-fidelity, reliable results, modifying portrait lighting and perspectives at photographic quality. 
	We further showcase it can be coupled with animation and style transfer tools to create vivid free-view styled facial animations.
\end{abstract}


==> section/depre/intro_deprecated.tex <==

\wz{
Consider that the results are still in progress, now we may claim it as an application paper? Specifically, I want to claim it as a 3D aware style transfer paper.  Currently I sell the story from the perspective of reconstruction, should focus more on style transfer/normal.

% motivation
1) style transfer is great, but mostly addressed in 2D. We address the 3D aware style transfer, not only transfer style, but also transfer the view and lighting. Note: Why this task is important? Should refer to the style transfer papers.  Also, relighting may be mentioned in a better way. 

% previous work limitation
2) It is a non-trivial task. View/lighting transfer requires 3D understanding --> Reconstruction tasks get explicit 3D, but generally hard to address hair and ears, let alone clothing, background 
Generation tasks could align view, rotate face in a more consistent way, but cannot enable photorealistic relighting. Moreover, invertion has problems. Note: need to verify PTI don;t work. If it works, we should write it in another way.

% observation
3) Our approach: utilize normal information to help both view transfer and lighting transfer. a. normal helps create a better 3D model and our fusion method gets better rendering results in other views.  b.normal is necessary in lighting transfer.  Note: This is very tricky. Currently, the novelty only happens in the 3D reconstruction part(normal based fusion). The lighting is totally achieved by IJCV. I think we can focus more on the pipeline it self.  Also, I think we have to make the styletransfer process stable for lighting. Think about how the normal can help here.

4. Applications: Non-photorealistic rendering, show we render image within arbitrary view/lighing and relighting.  
Note: Do we only support for front view input?  If so, we should lower down the claim...  
Also, Jingyi mentioned a lot of applications, how could we merge those within current pipeline?
}

\begin{comment}

% 1) why style tranfer is important?
% it seems I put the motivation to face photo to potraint paiting, is it true?
As a popular genre in the art world, portrait paintings present human faces with artists' creativity and imagination. Artists have created strong personal styles in the past hundreds of years, ranging from Da Vinci's Mona Lisa to Rembrandt's Self-Portraits. While it is impossible to draw new paintings from the % departed
historical artists, recent style transfer works demonstrate we can adopt neural methods to turn a face photo into a portrait painting with selected artist styles~\cite{gatys2015neural,johnson2016perceptual,selim2016painting}. Such techniques draw a lot of attention % become quite popular 
and inspire a series of popular industrial applications such as Prisma, Pikazo, DeepArt and Microsoft Pix~\cite{}.

Despite the cool effects previous works have achieved, most of them treat style transfer as an image to image translation problem and transfer image style in 2D space. However, images, especially photos or photorealistic paintings, are 2D projections of 3D geometry interacting with light. Famous portrait paintings, like Mona Lisa,  have unique face view and exquisite lighting effects. Due to lacking 3D understanding, existing works always transfer styles under fixed input views and ignore the lighting effects, which limits the usage of style transfer.

In this paper, we aim for a more challenging problem: 3D aware portrait stylization. 
Our goal is to transfer not only styles, but also view directions and illumination effects. 
E.g., assume we want to stylize a photo of Michael Jackson to Mona Lisa. Besides the  oil painting style, we are interested in transferring its pose and light to the same view direction and illuminate condition as Mona Lisa, as if Da Vinci replaced his model to Michaels Jackson.
Such a task provides more freedom to portrait stylization and enables numerous applications in virtual cinematography, movie post-production, visual effects and telepresence, so on and so forth.
\wz{we only take front face images as input? The last sentence is copied from existing words. It is a little verbose. We can further condense}

% 2) the task needs 2 modules, cannot be done by any previous work
% reocnsturciton based methd
% it seems I put the motivation to face photo to potraint paiting, is it true?
Portrait stylization under novel view and lighting is a non-trivial task, which composes of novel view synthesis, relighting and stylization. Furthermore, the input is limited to a single view face image, which makes this problem even more challenging. 
Rendering photorealistic novel views from a single image requires 3D face reconstruction. %understand the 3D information of a single view face image has 
As a long standing goal in computer vision and graphics, early methods rely on sophisticated devices~\cite{}. Recent neural network based 3DMM models~\cite{} produce faithful shape and texture for the main region of the face, but still limited to model complex corner cases, such as various hair styles, additional topology like glasses or ears, wrinkled clothes, as well as the background. As such, it fails to create photography quality, consistent novel views. %Recently, 3D generative models show promising results. We follow this line to inverse the   
On the other hand, existing stylization methods generally adopt CNN structure and address style transfer in 2D image space~\cite{}, which consider neither view alignment nor lighting consistency. Consequently, it produces undesirable results when encountering input images with huge view and lighting deviations. \wz{Is it ture? Can we do a user study?}
To the best of our knowledge, there hasn't been a mature solution to address all the components.

\wz{where is normal???}
In this paper, we propose to 
\end{comment}


==> section/depre/method1-view.tex <==

\section{Methodology}
\label{sec:overview}

{\ourmodel} stylizes a portrait with user desired perspective and lighting effects, producing novel view relit images with high photorealsm. 
We provide an overview of our method in Fig.~\ref{fig:overview}. 
Given a portrait input, {\ourmodel} sequentially modify its perspective and lighting effects. 
Finally we stylize and animate the edited images, generating movie special effects videos. \wz{application is unclear!}
%
We first describe photorealisitc free view synthesis in Sec.~\ref{sec:perspective}, then talk about our relighting module in Sec.~\ref{}. Lastly, we present style transfer and facial animation applications in Sec.~\ref{}.



\subsection{Photorealisitc Free View Synthesis}\label{sec:perspective}

% 对于给定一张RGB图像 I ，以及一个新的视角 V，我们希望得到对应视角下的RGB图像，以及surface normal，以供后续application使用。

% 如 fig.overview 展示，我们使用了两种方法，分别得到对应视角下的整体图像I_V^H 与 细节更为丰富、准确的面部图像 I_V^F 。并通过fusion的方法将二者融合，得到最终的效果。

% 对于整体图像，我们寻找StyleSDF的latent space，并根据输入图像进行fine-tune，以得到input image对应的SDF，以及可以生成任意变换视角的图像。

% 对于面部图像，我们使用细节丰富、准确的surface normal预测模组进行估计，并根据整体的SDF的深度作为先验进行Poisson normal integration，从而得到面部的mesh，用以进行新视角下的投影。

Take a portrait as input $\image$, our goal is to synthesize its novel view $\imageNote{\view}$ under a new view $\view$ in a realistic manner. % We further infer its surface normal map $\normalNote{\view}$ at $\view$, which is prepared for the relighting module and subsequent applications.
%
As shown in Fig.~\ref{fig:overview} (a), we first leverage the powerful geometry aware generative models~\cite{orel2021styleSDF}, applying GAN inversion~\cite{roich2021pivotal} to reverse the input to the latent code. The generator then map it to a coarse geometry and employ neural rendering to synthesize a high resolution novel view image $\imageNoteUp{\view}{\neural}$. We describe this part in Sec.~\ref{sec:invertion}

However, we observe that both inversion and neural rendering introduce artifacts in novel view synthesis, creating over-smoothed and aliasing results. As such, we further propose to enhance it with normal maps. Specifically, we employ a normal estimation network(Sec~\ref{}) to acquire an accurate normal map $\normal$ from the input $\image$. With the assistance of $\normal$, we improve the generated coarse geometry through Poisson normal integration~\cite{bibid}, producing a high quality mesh. We then texture it with the original image and render a new image $\imageNoteUp{\view}{\mesh}$.
Finally, we fuse $\imageNoteUp{\view}{\neural}$ and $\imageNoteUp{\view}{\mesh}$ and with Poisson blending~\cite{bibid}, generating a photorealistic image with minimal artifacts. We detail the mesh generation  and fusion  in Sec Sec, respectively.

% （删掉）对于给定的一张RGB图像，我们使用PTI inversion，得到其对应的stylesdf模型，与对应的latent。这一部分可以提供基于stylesdf框架的coarse geometry，free-view portrait以及对应视角的normal。


% （删掉）由于基于stylesdf的free-view portrait相比原图会有画质降低、xxx、xxx等问题，并且在基于style to radiance的生成框架下，inversion会导致生成时存在模糊、新视角下artifact等现象。尤其在人脸的区域内，这一现象更加明显。因此我们对人像的脸部使用了更加稳定的基于mesh的投影，得到细节更加稳定，清晰度更高的新视角图像。








% 整体人像生成
\subsection{Overall Image Generation}


% StyleSDF生成框架是一个基于Volume Rendering与上采样模块的3D-aware GAN生成器。其生成器包含一组参数theta，并以一个latent z ，一个noise n以及一个视角v作为输入。其对应输出为一张人像图，记作（公式）。此外，我们还可以获得空间中每一个voxel的density，用以后续计算normal与depth。
The StyleSDF generation framework is a 3D-aware GAN generator based on Volume Rendering with an upsampling module. The generator contains a set of parameters $\theta$ and takes a latent $\mathbf{z}$, a noise $\mathbf{n}$ and a viewpoint $\mathbf{v}$ as input. The output is a portrait image, denoted as $G(\mathbf{z}, \mathbf{n}, \mathbf{v} ;\theta)$. In addition, we can obtain the density of each voxel, which can be used for the subsequent calculation of normal and depth.
\wyj{Should we provide more details about StyleSDF?}


% 对于一张Input的图像，我们希望能够用StyleSDF的框架生成其其他视角的图像，并获得其三维几何。受到PTI的启发，我们通过两个阶段来完成这一目的。
For an image of an Input, we want to be able to use the framework of StyleSDF to generate images of its other views and to obtain its 3D geometry. Inspired by PTI, we do this in two stages.

% 第一个阶段为优化latent，noise与视角，为fine-tune过程提供一个好的起始条件。在这一个阶段中，我们锁定网络的参数，并优化上述三个变量。我们使用pcpt error与mse error来监督网络生成的图像，使其接近原图。此外，为了防止noise vector带来其他视角的artifact，我们引入了regular term。这一步的优化定义如下：公式。
The first stage is to optimise the latent, noise and perspective to provide a good starting condition for the fine-tune process. In this phase, we lock the parameters of the network and optimise the three variables mentioned above. We use pcpt error and mse error to monitor the images generated by the network so that they are close to the original image. In addition, to prevent the noise vector from bringing in artifacts from other perspectives, we introduce regular term. the optimisation for this step is defined as follows: 
\begin{equation}
    \mathbf{v}^*, \mathbf{z}^*, \mathbf{n}^* = \arg \min_{\mathbf{v}, \mathbf{z}, \mathbf{n}} \mathcal{L}_{mse}(I, G(\mathbf{v}, \mathbf{z}, \mathbf{n})) + \mathcal{L}_{pcpt}(I, G(\mathbf{v}, \mathbf{z}, \mathbf{n})) + \lambda L_{2}(\mathbf{n})
\end{equation}
\wyj{this paragraph seems like PTI. }

% 第二个阶段是finetune stylesdf的生成器。在这一步中，我们解锁网络的参数，并锁定xxx。在这一阶段，我们不仅要保证stylesdf生成的人像与原图更加接近，还要保证在视角变换时，一致性不被破坏。因此我们分别使用两个Loss来约束网络并进行训练。
% Tuning loss 通过计算输入的图像与生成的图像的差异，从而约束网络学习输入的图像特征，使得生成的人物与输入的人物接近。（公式）
% Regularization loss 通过在latent附近采样，并在任意视角下约束fine-tune后的网络生成的结果与原始网络生成的结果想接近，以保证图像的一致性不被破坏。（公式）
The second stage is the fine-tune StyleSDF generator. In this step we unfreeze the parameters $\theta$ of the network and freeze $\mathbf{v}^*, \mathbf{z}^*, \mathbf{n}^*$. In this stage we not only want to make the generated image is closer to the original image, but also keep the consistency when change the viewpoint. We therefore use two separate loss functions to train the network.
Tuning loss make the network to learn the input image features by calculating the difference between the input image and the generated image: 
\begin{equation}
     \mathcal{L}_{tune}(\theta) = \mathcal{L}_{mse}(I, G(\mathbf{v}^*, \mathbf{z}^*, \mathbf{n}^*; \theta)) + \mathcal{L}_{pcpt}(I, G(\mathbf{v}^*, \mathbf{z}^*, \mathbf{n}^*; \theta))
\end{equation}
Regularization loss ensures that the consistency of the images is not broken by sampling around the latent and constraining the fine-tuned network to generate results that are close to those generated by the original network at any viewpoint. 
\begin{equation}
\begin{aligned}
    \mathcal{L}_{reg}(\theta, \theta_0) &= \mathcal{L}_{mse}(G(\mathbf{v}_r, \mathbf{z}_r, \mathbf{n}_r; \theta_0), G(\mathbf{v}_r, \mathbf{z}_r, \mathbf{n}_r; \theta))\\ &+ \mathcal{L}_{pcpt}(G(\mathbf{v}_r, \mathbf{z}_r, \mathbf{n}_r; \theta_0), G(\mathbf{v}_r, \mathbf{z}_r, \mathbf{n}_r; \theta)),
\end{aligned}
\end{equation}
where $\theta_0$ is the network's weight before tunining, $\mathbf{z}_r$ is the interpolated code obtained by the interpolation method of [xxxPTI], $\mathbf{n}_r$ and $\mathbf{v}_r$ is randomly sampled in the training domain.
% 我们的优化目标是使得上述两个Loss达到最优，以得到最为合适的网络权重：
Our optimization objective is to optimize the above two Losses in order to obtain the most appropriate network weights $\theta^*$:
\begin{equation}
    \theta^* = \arg \min_{\theta} \mathcal{L}_{tune}(\theta) + \mathcal{L}_{reg}(\theta, \theta_0)
\end{equation}
%

% 1. Inversion
% （删掉）对于StyleSDF的生成框架，给定一组网络参数xxx，其input由两部分组成：latent z 与 noise。为了生成与input图像的人物特征一致的人像，我们根据PTI提出的方法，我们在StyleSDF的框架上进行了实现。这一过程分为两个步骤：优化camera pose, latent z 与 noise，与finetune 网络。
% 在优化latent z阶段，我们固定stylesdf的生成器参数，并以一组latent与noise作为起点进行优化。优化过程中，我们使用xxx loss与xxx loss进行监督。（公式xxx）。
% 与PTI不同的是，我们在这里使用了latent z 而不是latent w。这样做的原因是3D gan需要很强的多视角一致性。直接优化W将会脱离stylesdf训练的domain，导致在视角变换时失真。

% （删掉）第二个步骤是finetune网络。我们锁定上一步优化时使用的latent与noise，并解锁stylesdf的生成器参数。这一步中，我们使用两个loss进行优化：pivotal loss与local regularization loss。
% 作用，视角。



\subsection{Face Mesh}
% 对3D-aware的styleSDF进行inversion的过程中，会导致生成的图像高频信息丢失，并且三维一致性变差。由于在分辨人像identity时，面部细节十分重要，因此这一现象在人脸处更为明显。为了解决这一问题，我们使用了清晰度、保真度更高的Surface normal predictor对面部几何进行了预测。
% Surface Normal Predictor是一个U-net结构的神经网络。其输入是一张RGB人像图，输出是这张图片对应的Surface Normal。我们使用OLAT数据提供训练pair进行有监督训练。（这里需不需要具体写怎么构建的训练对？因为total里面写过，ijcv也写过。）
The process of inversion of a 3D-aware styleSDF results in a loss of high-frequency information in the resulting image and a deterioration in 3D consistency. This phenomenon is more pronounced at the human face because of the importance of facial detail when discriminating between portrait identities. To solve this problem, we have used the Surface normal predictor, which has higher definition and fidelity, to predict facial geometry.
The Surface Normal Predictor is a neural network with a U-net structure. The input is an RGB portrait image, and the output is the corresponding Surface Normal image. \wyj{Do we need to write exactly how the training pair is constructed here? Because it is written in total relighting and also in IJCV.}

% 通过积分Normal，我们可以恢复出人像面部的几何。但由于在一些地方，面部深度是非连续的（比如鼻子、嘴巴），因此在使用泊松积分时会有奇异性，面部几何会呈现扁平的效果。因此，我们引入上一步的人像SDF，为积分提供depth先验。
% 具体来说，我们首先通过xxx勾勒出人像的轮廓。在轮廓上，我们使用通过SDF的depth作为泊松积分的先验。然后，我们在面部区域使用泊松normal integration，得到最终的面部几何。
By integrating Normal, we can recover the geometry of the portrait face. However, since in some places the facial depth is incontinuous (e.g. nose, mouth), there will be ambiguity when using Poisson integration and the facial geometry will take on a flattened effect. Therefore, we introduce the portrait SDF from the previous step to provide a depth prior for the integration.
Specifically, we first outline the portrait through xxx. On the outline, we use the depth through the SDF as a prior for the Poisson integration. We then use Poisson normal integration in the face region to obtain the final face geometry.
\wyj{should we introduce Poisson integration equation here?}

% 通过上一步求得的拍摄角度，我们可以对几何进行重投影，得到每个节点在原图上的坐标。我们将投影的坐标视作节点的texture坐标，并使用原图或normal的图像作为面部mesh的texture map，以支持新视角下的投影。
Using the shot view obtained in the previous step, we can reproject the geometry to obtain the coordinates of each node on the original image. We treat the projected coordinates as the texture coordinates of the nodes and use the original or normal image as the texture map of the facial mesh to support the projection in the new perspective.

% 2. Face Mesh
% （删掉）为了解决面部细节丢失等情况，我们接下来通过基于mesh的重新投影的方式得到更高清晰度、更稳定的人脸。为了得到高保真度的几何，我们使用了基于surface normal的方法，并将stylesdf的几何作为先验。
% 具体来说，我们首先训练了一个rgb portrait image to surface normal的网络。这一网络的核心结构是U-net。在训练中，我们使用有监督学习，并通过OLAT数据集构建training pairs。使用这一网络，我们可以得到input image对应的surface normal。
% （删掉）直接使用surface normal进行积分会导致xxx的现象（需要reference）。因此我们使用xxx勾勒出人物的五官轮廓与面部区域，并将轮廓上的stylesdf的depth作为积分边界。通过这样的方法，我们可以得到细节分明，且符合人物特征的几何（mesh）。
% 我们使用原图作为texture map，并根据mesh在原图上的投影位置设定mesh的vt坐标。

\subsection{Fusion}
% 对于任意给定的新视角，我们期望得到一个高质量的人像，以及对应视角下的normal，以实现后续relighting、stylization等操作。

% 对于RGB图像，我们首先使用fine-tune的生成器以及latent，我们可以渲染出包含背景、头部与身体的完整的人像。然后，我们使用面部的mesh以及对应的贴图，在新的视角下进行投影，得到细节丰富、准确的面部图像。
% 我们使用泊松图像融合的方法将二者融合，以生成最终的图像

% 对于Normal图像，我们使用fine-tune的生成器以及latent求得每个voxel的density，并对其求导得到每个voxel的法向，再通过积分的方式得到每个pixel对应的surface normal。面部的normal与RGB的投影方式类似，但在投影前需要先进行一步方向变换。
For any given new viewpoint $\mathbf{v}_n$, we expect a high quality RGB portrait image and a normal image for the corresponding viewpoint for subsequent relighting, stylisation etc.

For the RGB image, we first use the fine-tune generator $G(\theta^*)$, the latent $\mathbf{z}^*$ and the noise $\mathbf{n}^*$, which allows us to render a complete portrait with background, head and body. We then use the mesh of the face $M$ to project on a new perspective to obtain a detailed and accurate image of the face.
We fuse the two images by Poisson image blending method to produce the final image.

For the Normal image, we use the fine-tune generator and latent to find the density of each voxel, calculate the normal of each voxel $\mathbf{x}$ as $\mathbf{n}(\mathbf{x}) = \nabla \sigma(\mathbf{x})$
and then integrate to obtain the surface normal for each pixel by the volume rendering equation of SDF.
The normal of the face is similar to the RGB projection, but a step of directional transformation is required before projection.


% 3. Fusion
% （删掉）对于任意给定的新视角，我们期望得到一个高质量的人像，以及对应视角下的normal，以实现后续relighting、stylization等操作。对于一个给定的视角，我们分别通过stylesdf渲染人像，通过mesh渲染人脸。我们使用泊松图像融合的方式将两者进行融合，以保证边缘的连续性。与之类似，我们通过xxx的方式的方式得到stylesdf在对应视角下的normal，并与面部的normal进行融合。


\subsection{religting}
Lighting is fundamental to one's feeling of a portrait image. 
We utilize a relighting module inspired by~\cite{pandey2021total} to achieve high-fidelity portrait lighting editing. The relighitng module consists of albedo network, normal network and a relighting network. We first use the albedo network to extract the albedo under each viewpoint. 

We train a U-net structure network to achieve relighting effect, and use the Phong shading as prior. In details, for a given target illumination, we use Phong shading to render the diffuse light map and four specualr light maps with different shininess exponents, as the input of the relighting network. The output of the network is the final portrait under target illumination.
To train the network, we use Dynamic-OLAT (one-light-at-time) dataset [xxxNVPR] as training set for supervised learning.

Different from~\cite{pandey2021total}, our normal map for Phong shading is not generated by per-frame prediction. Instead, we propose a novel fused normal map, which has 3D consistent property.  For free-view video relighting, the fused normal map produces a more stable and consistent shading prior to the relighting network.

% 1. lighting
% 

% 受到[total relighting]的启发，我们的relighting模块首先使用albedo prediction network提取每个视角下的albedo。对于一个给定的光照，我们首先使用phong shading进行预渲染，为relighting module提供先验。我们渲染了diffuse与四种材质下的specular，作为5*3个通道的input输入到relighting network。relighting network是一个u-net结构的网络，并使用olat数据作为训练数据，进行有监督学习。相比total relighting，我们的normal使用了更加稳定的fusion normal，而不是逐帧进行预测，因此在视频中会有个更加稳定、一致






\subsection{Motion}


% 3. annimation


% liminzhang：
%
%这个应用下，给定一个指定的对象S，标记它在不同视角下的图像，S^v。我们的目标是用驱动帧D_t去独立地处理S^v，获得S^v_t，使得S^v_t具有D_t的相对运动信息以及S的内容信息，同时维持v变化时和t变化时S的几何一致。为实现这个目的，我们采用fomm的驱动流程。

% fomm由两部分组成，动作生成模块和图像生成模块。动作生成模块是为了预测dense motion field，这个field包含了驱动帧D_t（3XHXW）和原图S^v之间像素位置的映射关系，被T_(S<-D)建模。[?]图像生成模块接受dense motion field和原图做输入，生成具有运动信息的S^v_t.[?]

% 基于fomm，我们的驱动阶段具体分成三个阶段。
% 首先，D和S中关键点的位置分别由一个编码器-解码器网络预测。关键点检测器网络输出关键点位置以及每个仿生变换的参数。

% 之后，密集运动网络结合了局部近似值，得到了所产生的密集运动场T(S^v←D_t)。在这里，我们和fomm在encode相对运动时采用了不同的估计策略。fomm的做法是将D1到Dt的变换作用在S^v上，但这assume S^v和D1有相近的pose。在我们的case下，我们先生成和D1的pose一致的新视角图片S^p(D1)与该视角图片到目标视角的FVV，然后分别通过网络估计Dt到D1的 变换，并解算T(S^p(D1)_1<-Dt)[?]和T(S^v <- S^p(D1)).得到变换T（S^v_1 <- S^v_t）。这种策略背后的直觉是NAPSTER出的的脸部特征在3D网格空间几何一致，使得新视角生成图像自然适用于fomm的驱动范式。因此NAPSTER即使是新视角pose和驱动视频不一致，也能够借由FVV解算出的变换，comparably达到特效级别的驱动结果。

%最后，生成模块渲染源物体移动的图像。使用一个生成器网络G，根据TˆS←D对源图像进行扭曲，并对源图像中被遮挡的部分进行预测。

Under this application, given a specified object S, mark its image at different viewpoints, $S^v$. Our goal is to process $S^v$ independently with the drive frame $D_t$ to obtain $S^v_t$ such that $S^v_t$ has the relative motion information of $D_t$ as well as the content information of S, while maintaining the geometric consistency of S when v changes and when t changes. To achieve this, we use the driving process of fomm.

The fomm consists of two parts, the motion generation module and the image generation module. The motion generation module is designed to predict the dense motion field, which contains the mapping relationship of pixel positions between the driving frame $D_t$(3XHXW) and the original image $S^v$, modeled by $T_(S<-D)$. [?] The image generation module accepts the dense motion field and the original image as input to generate $S^v_t$ with motion information.[?]


Based on fomm, our drive phase is specifically divided into three stages.


First, the locations of keypoints in D and S are predicted by an encoder-decoder network, respectively. The keypoint detector network outputs the keypoint positions and the parameters of each affine transformation.



\subsection{Style}
% 我们做了两种风格迁移，作为我们的application。
% 第一种是生成中世纪油画的风格。（不确定是不是中世纪）。
% 为了实现人物identity一致的风格迁移，我们使用pix2pix作为生成框架，并构建训练pair作为训练数据。为了构建人物identity一致的训练pair，我们首先使用“Awesome Pretrained StyleGAN”生成了50000张油画。这些油画被用来fine-tune 在ffhq上预训练好的stylegan。在fine-tune的过程中，我们固定stylegan的前几层，只训练最后两层，这样可以保证人像与油画的identity一致。然后我们通过在fine-tune前的和fine-tune后的网络，使用相同的latent进行生成，即可得到一组training pair。

% https://github.com/justinpinkney/awesome-pretrained-stylegan

% 通过这个pix2pix的网络，我们可以生成一张图像对应的油画风格。此外，由于我们还拥有这张图像对应的normal，因此可以进行进一步的光照编辑。具体做法是，我们用sec.relighting的方法，对原图进行relighting，并与原图相除计算shading map。将shading map乘以风格化后的结果，得到relighting后的油画



% 另一个应用是hatching。在素描中，笔触往往与两方面有关：亮度与几何结构。亮度往往控制线条的疏密，而几何结构影响了线条的走向。我们的工作可以同时生成表达亮度信息的RGB图像与表达几何信息的Normal。使用Kim 等人的工作，我们可以将一个视角下的RGB图像与Normal转化成素描的风格。

% Line-art Illustration of Dynamic and Specular Surfaces 



% - Pix2pixHD, enabling style transfer(油画) with (roughly) pixel alignment. 





% - Style Transfer with lighting change (normal assisted). 





% - Hatching styles(normal is used, lighting, sketch directions). 




